MA-DST: Multi-Attention Based Scalable Dialog State Tracking

Task oriented dialog agents provide a natural language interface for users to complete their goal. Dialog State Tracking (DST), which is often a core component of these systems, tracks the system's understanding of the user's goal throughout the conversation. To enable accurate multi-domain DST, the model needs to encode dependencies between past utterances and slot semantics and understand the dialog context, including long-range cross-domain references. We introduce a novel architecture for this task to encode the conversation history and slot semantics more robustly by using attention mechanisms at multiple granularities. In particular, we use cross-attention to model relationships between the context and slots at different semantic levels and self-attention to resolve cross-domain coreferences. In addition, our proposed architecture does not rely on knowing the domain ontologies beforehand and can also be used in a zero-shot setting for new domains or unseen slot values. Our model improves the joint goal accuracy by 5% (absolute) in the full-data setting and by up to 2% (absolute) in the zero-shot setting over the present state-of-the-art on the MultiWoZ 2.1 dataset.

==> dataset.tex <==
We evaluate our approach on MultiWOZ, a multi-domain Wizard-of-Oz dataset. MultiWOZ 2.0 is a recent dataset of labeled human-human written conversations spanning multiple domains and topics \cite{budzianowski-etal-2018-multiwoz}. As of now, it is the largest labeled, goal-oriented, human-human conversational dataset with around 10k dialogs, each with an average of 13.67 turns. The data spans seven domains and 37 slot types. Due to patterns of annotation errors found in MultiWOZ 2.0, \cite{ericMultiWOZ21} re-annotated the data and released a MultiWOZ 2.1 version, which corrected a significant number of errors. Table \ref{newDataStats} mentions the percentage of slots in each domain whose values changed with the MultiWOZ 2.1 re-annotation. 

For all our experiments, we use MultiWOZ 2.1 data, which is shown to be cleaner and more challenging because many slots are now correctly annotated with their corrected values or $dontcare$ instead of $none$. We are using only five domains out of the available seven - namely $(\text{restaurant}, \text{hotel}, \text{attraction}, \text{taxi}, \text{train})$ - since the other two domains $(\text{bus}, \text{police})$ are only present in the training set. We use the provided train/dev/test split for our experiments. 
    
\begin{table}[h!]
\centering
\begin{tabular}{p{1cm} p{1.5cm}  p{1cm} p{1cm} p{1cm} p{1cm}}
 \multicolumn{6}{c}{Slot Values Updated in MultiWOZ 2.1} \\
   & Restaurant & Taxi & Hotel & Train & Attraction\\
 \hline
 Train  & 13.64 & 3.65 & 26.89 & 7.04  & 12.69\\
 Dev    & 22.04 & 3.18 & 20.93 & 5.88  & 12.82\\
 Test   & 19.33 & 3.95 & 24.70 & 10.59 & 16.12\\
  \hline
 \end{tabular}
 \caption{Percentage of slot values that changed in MultiWOZ 2.1 compared to MultiWOZ 2.0. }
 \label{newDataStats}
\end{table}


==> relatedWork.tex <==
Dialog state tracking (DST) is a core dialog systems problem that is well studied in the literature. Earlier approaches for DST relied on Markov Decision Processes (MDPs)~\cite{levin2000stochastic} and partially observable MDPs (POMDPs)~\cite{williams2007partially,Thomson:2010} for estimating the state updates. See \cite{williams2016the} for a review of DST challenges and earlier related work.

%Such systems leverage information from language understanding \cite{williams-2014-web} and speech recognition output \cite{henderson-etal-2014-word}. 

Recent neural state tracking approaches achieve
state-of-the-art performance on DST \cite{gao2018neural}. Some
of this work formulates the state tracking problem as a classification task over
all possible slot-values per
slot \cite{mrksic-etal-2017-neural,wen-etal-2017-network,liuLane2017}. This
assumes that an ontology containing all slot values per slot is available in
advance. In practice, this is a limiting assumption, especially for free-form
slots that may contain values not seen during training \cite{xu-hu-2018-end}. To

address this limitation, \cite{46399} propose a candidate generation approach
based on a bi-GRU network, that selects and scores slot values from the
conversation history. \cite{xu-hu-2018-end} propose using a pointer
network \cite{NIPS2015_5866} for extracting slot values from the
history. More recently, hybrid approaches which combine the candidate-set
and slot-value generation approaches have appeared~\cite{goel2019hyst,trade2019}. 

Our work is most similar to TRADE~\cite{trade2019}, and extends it by proposing
self~\cite{cheng-etal-2016-long} and
cross-attention \cite{BahdanauCB14} mechanism for
capturing slot and history correlations. Attention based archirectures like the
Transformer \cite{Vaswani:2017} and architectures that extend it, like
BERT \cite{devlin-etal-2019-bert} and RoBERTa \cite{roberta}, achieve the
current state-of-the-arts for many NLP tasks. We are also inspired by the work in
reading comprehension where cross attention is used to compute relations between
a long passage and a query question \cite{zhu2018sdnet,Chen_2017}.

For benchmarking, DSTC challenges provide a popular experimentation framework
and dialog data collected through human-machine interactions. Initially, they
focused on single domain systems like bus routes \cite{WilliamsRRB13}. Wizard-of-Oz (WOZ) is also a
popular framework used to collect human-human dialogs that reflect the target
human-machine behavior \cite{wen-etal-2017-network,asri2017frames}. Recently,
the MultiWOZ 2.0 dataset, collected through WOZ for multiple domains, was
introduced to address the lack of a large multi-domain DST
benchmark \cite{budzianowski-etal-2018-multiwoz}. \cite{ericMultiWOZ21} released
an updated version, called MultiWOZ 2.1, which contains annotation corrections
and new benchmark results using the current state-of-the-art approaches. Here, we use the MultiWOZ 2.1
dataset as our benchmark.




